AdSplit: Separating smartphone advertising from applications

A wide variety of smartphone applications today rely on third-party advertising services, which provide libraries that are linked into the hosting application. This situation is undesirable for both the application author and the advertiser. Advertising libraries require additional permissions, resulting in additional permission requests to users. Likewise, a malicious application could simulate the behavior of the advertising library, forging the user's interaction and effectively stealing money from the advertiser. This paper describes AdSplit, where we extended Android to allow an application and its advertising to run as separate processes, under separate user-ids, eliminating the need for applications to request permissions on behalf of their advertising libraries. We also leverage mechanisms from Quire to allow the remote server to validate the authenticity of client-side behavior. In this paper, we quantify the degree of permission bloat caused by advertising, with a study of thousands of downloaded apps. AdSplit automatically recompiles apps to extract their ad services, and we measure minimal runtime overhead. We also observe that most ad libraries just embed an HTML widget within and describe how AdSplit can be designed with this in mind to avoid any need for ads to have native code.

==> abstract.tex <==
% \todo[inline]{Written by Mike, have Shashi and Dan remove/rewrite}
A wide variety of smartphone applications today rely on third-party advertising services, which provide libraries that are linked into the hosting application. This situation is undesirable for
both the application author and the advertiser. Advertising libraries require additional permissions, resulting in additional permission requests to users. Likewise, a malicious application could simulate the behavior of the advertising library, forging the user's interaction and effectively stealing money from the advertiser. This paper describes \projname, where we extended Android to allow an application and its advertising to run as separate processes, under separate user-ids, eliminating the need for applications to request permissions on behalf of their advertising libraries.
We also leverage mechanisms from \quire to allow the remote server to validate the authenticity of client-side behavior. In this paper, we quantify the degree of permission bloat caused by advertising, with a study of thousands of downloaded apps. \projname automatically recompiles apps to extract their ad services, and we measure minimal runtime overhead. We also observe that most ad libraries just embed an HTML widget within and describe how \projname can be designed with this in mind to avoid any need for ads to have native code.

% Smartphone apps and the advertisement libraries that monetize them often run within the same code base.  This situation requires that apps request permissions on behalf of the ad libraries they host, even when those permissions are unused by the app itself.  These permissions, used only by hosted ad libraries, increase the permission bloat of the app and can be used for nefarious purposes by an untrustworthy ad library.  In \projname, we engineered a method for splitting the main app from the ad libraries it hosts while introducing a trusted path mechanism to the smartphone user interface that allows the ad libraries to validate user input.  \projname allows an application and advertisements to run in separated isolated application domains. This allows ad libraries to be isolated and have their own permission sets.  We demonstrate the usefulness of \projname by examining two app stores to determine the permission reductions afforded by this approach.  We further show that the performance overhead of \projname is minimal by analyzing the communication and memory overhead of our modifications. 


==> ack.tex <==
\section*{Acknowledgements}
This work builds on our prior \quire project. We thank Yuliy Pisetsky and Anhei Shu for their assistance and efforts.
This work was supported in part by NSF grants CNS-1117943 and CNS-0524211.



==> conclusion.tex <==
\section{Conclusion}

We have presented \projname, an Android-based advertising system that
provides advertisers integrity guarantees against potentially hostile
applications that might host them. \projname leverages several
mechanisms from \quire to ensure that UI events are correct and to
communicate to the outside world in a fashion that hosting
applications cannot forge.  \projname runs with marginal performance
overhead and, with our HTML-based design, offers a clear path toward
widespread adoption.  \projname not only protects advertisers against
click fraud and ad blocking, it also reduces the need for permission
bloat among advertising-supported free applications, and has the
potential to reduce the incentive for applications to leak
privacy-sensitive user information in return for better advertising
revenues.


==> future_work.tex <==
\section{Future Work}

The work in this paper touches on a trend that will become
increasingly prevalent over the next several years: the merger of the
HTML security model and the smartphone application security model.
Today, HTML is rapidly evolving from its one-size-fits-all security origins to
allow additional permissions, such access to location information, for
specific pages that are granted those permissions by the user. HTML
extensions are similarly granted varying permissions rather than
having all-or-nothing
access~\cite{barth-extensions2010,liu-chrome-ndss2012}. 

On the flip side, iOS apps originally ran with full, unrestricted
access to the platform, subject only to vague policies enforced by
human auditors.  Only access to location information was
restricted. In contrast, the Android security model restricts the
permissions of apps, with many popular apps running without any
optional permissions at all. Despite this, Android malware is a
growing problem, particularly from third-party app stores (see,
e.g.,~\cite{Felt:2011:SMM,DroidRanger2012}). Clearly, there's a need
for more restrictive Android security, more like the one-size-fits-all
web security model.

While it's unclear exactly how web apps and smartphone apps will
eventually become one thing, our paper shows where this merger is
already underway: when web content is embedded in a smartphone app.
Well beyond advertising, a variety of smartphone apps take the
strategy of using native code to set up one or more web views, then
to the rest in HTML and JavaScript. This has several advantages: it
makes it easier to support an app across many different smartphone
platforms. It also allows authors to quickly update their apps,
without needing to go through a third-party review process.

These trends, plus the increasing functionality in HTML5, suggest that
``native'' apps may well be entirely supplanted by some sort of
``mobile HTML'' variant, not unlike HP/Palm's WebOS, where every app
is built this way\footnote{\url{http://developer.palm.com/blog}}. 

Maybe this will result in a industry battle royale, but it will also
offer the ability to ask a variety of interesting security questions.
For example, consider the proposed ``web intents''
standard\footnote{\url{http://webintents.org/}}. How can an
``external'' web intent interact safely with the ``internal'' Android
intent system? Both serve essential the same purpose and use similar
mechanisms. We, and others, will pursue these toward
interesting conclusions.


==> introduction.tex <==
\section{Introduction}

The smartphone and tablet markets are growing in
leaps and bounds, helped in no small part by the availability of
specialized third-party applications (``apps'').  Whether
on the iPhone or Android platforms, apps often come in two flavors: a
free version, with embedded advertising, and a pay version without.
Both models have been successful in the marketplace.  To pick one
example, the popular Angry Birds game at one point brought in roughly
equal revenue from paid downloads on Apple iOS devices and from
advertising-supported free downloads on
Android devices~\cite{angry-birds-wired}. They now offer advertising-supported
free downloads on both platforms.

We cannot predict whether free or paid apps will dominate in the
years to come, but advertising-supported
applications will certainly remain prominent. Already, a cottage industry of
companies offer advertising services for smartphone application
developers.

Today, these services are simply pre-compiled code libraries, linked
and shipped together with the application. This means that a remote
advertising server has no way to validate a request it receives from a
user legitimately clicking on an advertisement. A malicious
application could easily forge these messages, generating revenue for
its developer while hiding the advertisement displays in their
entirety. To create a clear trust boundary, advertisers would benefit
from running separately from their host applications.

In Android, applications must request permission at install time for
any sensitive privileges they wish to exercise. Such privileges
include access to the Internet, access to coarse or fine location
information, or even access to see what other apps are installed on
the phone. Advertisers want this information to better profile users
and thus target ads at them; in return, advertisers may pay more money
to their hosting applications' developers. Consequently, many
applications which require no particular permissions, by themselves,
suffer {\em permission bloat}---being forced to request the privileges
required by their advertising libraries in addition to any of their
own needed privileges. Since users might be scared away by detailed
permission requests, application developers would also benefit if ads
could be hosted in separate applications, which might then make their
own privilege requests.

And, of course, separating applications from their advertisements
creates better fault isolation. If the ad system fails or runs slowly, the host
application should be able to carry on without inconveniencing the
user.  Addressing these needs requires developing a suitable
software architecture, with OS assistance to make it robust. 

The rest of the paper is organized
as follows: first in Section~\ref{sec:analysis} we present a survey of thousands of 
Android applications, and estimate the degree of permission bloat caused by advertisement
libraries. Then in Section ~\ref{sec:web_ad_security} we discuss advertisement security on web
and the challenges for securing advertisements on smartphones. Section~\ref{sec:design}
describes the design of \projname,
Section~\ref{sec:implementation}  describes our Android-based
implementation, and
Section~\ref{sec:performance} quantifies its performance.
%
Section~\ref{sec:ad_separation} provides 
details about a simple binary rewriter  to adapt legacy apps to use our system. 
%
Section~\ref{sec:ad_newmodel} considers how we might eliminate native
code libraries for advertisements and go with a more web-like
architecture.
%
Finally, Section~\ref{sec:policy} discusses a variety of policy
issues.



\if 0
To that end, we first surveyed thousands of advertising-supported
Android applications to see which advertisement libraries are used and
to estimate the degree of permission bloat 
caused by the advertisement libraries (Section~\ref{sec:analysis}).
We then designed \projname, building on the \quire Android extension,
to allow advertising-supported applications to run separately, with
fewer privileges. XXX Section~\ref{sec:policy} discusses several
policy and user experience issues that would inevitably arise in any
attempt to commercialize \projname, such as how ad-blocking services
might be built (and how they might be defeated).
\todo[inline]{Section forward references}
\fi


==> macros.tex <==
\usepackage{todonotes}

\usepackage{amsfonts}
\usepackage{textcomp}
\usepackage{wasysym}

%PROJECT NAME MACRO
\usepackage{xspace}
\newcommand{\projname}{AdSplit\xspace} 
\newcommand{\quire}{\textsc{Quire}\xspace} 
\newcommand{\am}{{\em ActivityManager }}
\newcommand{\wm}{{\em WindowManager }}
\newcommand{\manifest}{{\em AndroidManifest.xml }}
\newcommand{\appframe}{{\em AppFrame }}
\newcommand{\pkgparser}{{\em PackageParser }}
\newcommand{\activityrecord}{{\em ActivityRecord }}
\newcommand{\taskrecord}{{\em TaskRecord }}
\newcommand{\adview}{{\em AdView }}
\newcommand{\motionevent}{{\em MotionEvent }}
\newcommand{\webview}{{\em WebView }}



==> policy.tex <==
\section{Policy}
\label{sec:policy}
While \projname allows for and incentivizes applications to run
distinct from their advertisements, there are a variety of policy and
user experience issues that we must still address.

\subsection{Advertisement blocking}
Once advertisements run as distinct processes, some fraction of the
Android users will see this as an opportunity to block advertisements
for good. Certainly, with web browsers, extension like AdBlock and
AdBlock Plus are incredibly popular. The Chrome web store lists
these two extensions in its top
six\footnote{\url{https://chrome.google.com/webstore/category/popular}}
with ``over a million'' installs of each. (Google doesn't disclose
exact numbers.)

The Firefox add-ons page offers more details, claiming
that AdBlock Plus is far and away the most popular Firefox extension,
having been installed just over 14 million
times, versus 7 million for the next most popular extension\footnote{\url{https://addons.mozilla.org/en-US/firefox/extensions/?sort=users}}.
The Mozilla Foundation estimates that 85\% of their users have
installed an extension~\cite{firefox-customized}. Many will install
an ad blocker.

To pick one example, Ars Technica, a web site popular with tech-savvy
users, estimated that about 40\% of its users
ran ad blockers~\cite{ars-technica-blockers}. At point, it added code to display
blank pages to these users in an attempt to cajole
them into either paying for ad-free ``premium'' service, or at least configuring their
ad blocker to ``white list'' the Ars Technica website.

Strategies such as this are perilous. Some users, faced with a broken
web site, will simply stop visiting it rather than trying to sort out
why it's broken. Of course, many web sites instead employ a variety of
technical tricks to get around ad blockers, ensuring their ads will
still be displayed.

Given what's happening on the web, it's reasonable to expect a similar
fraction of smartphone users might want an ad blocker if it was
available, with the concomitant arms race in ad block
versus ad display technologies.

So long as users have not ``rooted'' their phones, a variety of core
Android services can be relied upon by host applications to ensure
that the ads they're trying to host are being properly displayed with
the appropriate advertisement content.  Similarly, advertising
applications (or HTML ads) can make SSL connections to their remote
servers, and even embed the proper remote server's public key certificate, to ensure they are downloading data from the proper source,
rather than empty images from a transparent proxy.

Once a user has rooted their phone, of course, all bets are off.
While it's hard to measure the total number of rooted Android phones,
the CyanogenMod Android distribution, which requires a rooted phone
for installation, is installed on roughly 722 thousand
phones\footnote{\url{http://stats.cyanogenmod.com/}}---a tiny fraction
of the hundreds of millions of Android phones reported to be in
circulation~\cite{android-circulation-3q2011}. Given the relatively small
market share where such hacks might be possible, advertisers might
be willing to cede this fraction of the market rather than do battle against it.

Consequently, for the bulk of the smartphone marketplace, {\em
advertising apps on Android phones offer greater potential for blocking-detection
and blocking-resistance than advertising on the web}, regardless of
whether they are served by in-process libraries or by \projname. Given
all the other benefits of \projname, we believe advertisers and
application vendors would prefer \projname over the status quo.

\subsection{Permissions and privacy}

Some advertisers would appear to love their ability to learn
additional data about the user, including location information,
address book, other apps running on the phone, and so forth. This
information can help profile a user, which can help target ads.
Targeted ads, in turn, are worth more money to the advertiser and thus
worth more money to the hosting application. When we offer HTML style
advertisements, with HTML-like security restrictions, the elegance of
the solution seems to go against the higher value profiling that advertisers
desire.

Leaving aside whether it's {\em legal} for advertisers to collect this
information, we have suggested that a host application could make its
own requests that violate the users' privacy and pass these into the
\projname advertising app. We hope that, if we can successfully reduce
apps' default requests for privileges that they don't really need,
then users will be less accustomed to seeing such permission
requests. When they do occur, users will push back, refusing to
install the app. (Reading through the user-authored comments in the
Android Market, many apps with seemingly excessive permission
requirements will often have scathing comments from users, along with
technical justifications posted by the app authors to explain why each
permission is necessary.)

Furthermore, if advertisers ultimately prefer the \projname
architecture, perhaps due to its improved resistance to click fraud
and so forth, then they will be forced to make the trade-off between
whether they prefer improved integrity of their advertising platform,
or whether they instead want less integrity but more privacy-violating
user details.


==> related_work.tex <==
\section{Related Work}
\subsection{Web security}
\projname considers an architecture to allow for controlled mashups of
advertisements and applications on a smartphone. The web has been
doing this for a while (as discussed in
Section~\ref{sec:web_ad_security}). Additionally, researchers have
considered a variety of web extensions to further contain browser
components in separate
processes~\cite{op-webbrowser,isolation-chrome}, including
constructing browser-based multi-principal operating systems~\cite{howell2007mashupos,gazelle}.

\subsection{JavaScript sandboxes}
Caja~\cite{google-caja} and ADsafe~\cite{adsafe} work as JavaScript sandboxes which 
use static and dynamic checks to safely host JavaScript code. They use a safe subset
of JavaScript, eliminating dangerous primitives like {\tt eval} or
{\tt document.write} that could allow an advertisement to take over an
entire web page. Instead, advertisements are given a limited API to
accomplish what they need. \projname can trivially host advertisements
built against these systems, and as their APIs evolve, they could be
directly supported by out AdWebView class. Additionally, because we
run the AdWebView in a distinct process with its own user-id and
permissions, we provide a strong barrier against advertisement
misbehavior impacting the rest of the platform.

\subsection{Advertisement privacy}
Privad~\cite{nsdi11-privad} and Juels et~al.~\cite{privacy-target} address security issues related to
privacy and targeted advertising for web ads. They use client side software that prevents behavior profiling of 
users and allows targeted advertisements without compromising user privacy. 

\projname does not address privacy problems related to targeted advertisements but it provides framework for implementing 
various policies on advertisements. 

\subsection{Smart phone platform security}
As mobile phone hardware and software increase in complexity the
security of the code running on a mobile devices has become a major
concern.

The Kirin system~\cite{kirin} and
Security-by-Contract~\cite{SecbyC} focus on enforcing install time
application permissions within the Android OS and .NET framework
respectively.
These approaches to mobile phone security allow a user
to protect themselves by enforcing blanket restrictions on what
applications may be installed or what installed applications may do, but do little to protect the user from
applications that collaborate to leak data or protect applications
from one another.

Saint~\cite{saint} extends the functionality of the
Kirin system to allow for runtime inspection of the full system
permission state before launching a given application.
Apex~\cite{nauman2010apex} presents another solution for the same
problem where the user is responsible for defining run-time constraints on top
of the existing Android permission system.  Both of these approaches
allow users to specify static policies to shield
themselves from malicious applications, but don't allow apps to make dynamic
policy decisions.

CRePE~\cite{conti2011crepe} presents a solution that attempts to artificially restrict an
application's permissions based on environmental constraints such as
location, noise, and time-of-day.  While CRePE considers contextual
information to apply dynamic policy decisions, it does not attempt to
address privilege escalation attacks.

\subsubsection{Privilege escalation}
XManDroid~\cite{xmandroid} presents a solution for privilege escalation and
collusion by restricting communication at runtime between
applications where the communication could open a path leading to dangerous
information flows based on Chinese Wall-style
policies~\cite{brewer-nash-82} (e.g.,
forbidding communication between an application with GPS privileges and an
application with Internet access). While this does protect against some
privilege escalation attacks, and allows for enforcing a more flexible range
of policies, applications may launch denial of service
attacks on other applications (e.g., connecting to an application and thus
preventing it from using its full set of permissions) and it does not allow the 
flexibility for an application to regain privileges which they lost due to communicating
with other applications.
% In addition, while XManDroid identified two covert
% channels which they were able to protect, other channels may still exist to
% leak data. However, this approach does carry a lighter performance penalty
% compared to dynamic taint analysis.

One feature of \quire that is not used in \projname is its ability to 
defeat confused deputy attacks, by annotating IPCs with the entire
call chain.
In concurrent work to \quire, Felt et al. present a solution to what
they term ``permission re-delegation'' attacks against deputies on the
Android system~\cite{berkeley-ipc}. With their ``IPC inspection''
system, apps that receive IPC requests are poly-instantiated based on
the privileges of their callers, ensuring that the callee has no
greater privileges than the caller.  IPC inspection addresses the same
confused deputy attack as \quire's ``security passing'' IPC
annotations, however the approaches differ in how intentional deputies
are handled.  With IPC inspection, the OS strictly ensures that
callees have reduced privileges. They have no mechanism for a callee
to deliberately offer a safe interface to an otherwise dangerous
primitive.  Unlike \quire, however, IPC inspection doesn't require
apps to be recompiled or any other modifications to be made to how
apps make IPC requests.

(\projname does not require \quire's IPC inspection system, and thus also
does not require apps to be recompiled to have the semantics described
in this paper.)

More recent work has focused on kernel extensions that can observe
IPC traffic, label files, and enforce a variety of
policies~\cite{bugiel-android-ndss2012,seandroid2011}. These systems
can enhance the assurance of many of the above techniques by
centralizing the policy specification and enforcement mechanisms.

\subsubsection{Dynamic taint analysis on Android}
The TaintDroid~\cite{taintdroid} and
ParanoidAndroid~\cite{paranoidAndroid} projects present dynamic
taint analysis techniques to preventing runtime attacks and data
leakage.
These projects attempt to tag objects with metadata in order to track
information flow and enable policies based on the path that data
has taken through the system.  TaintDroid's approach to information
flow control is to restrict the transmission of tainted data to a
remote server by monitoring the outbound network connections made from
the device and disallowing tainted data to flow along the outbound
channels. 

\projname allows ads to run in separate processes but applications can still 
pass sensitive information to separated advertisements. TaintDroid and ParanoidAndroid
can be used to detect and prevent any such flow of information. Thus they are 
complementary to \projname.

\if 0
The goal of \quire differs from that of taint analysis in
that \quire is focused on providing provenance information and preventing
the access of sensitive data, rather than in restricting where data may flow.

The low level approaches used to tag data also differ between the
projects. TaintDroid enforces its taint propagation semantics by
instrumenting an application's DEX bytecode to tag every variable,
pointer, and IPC message that flows through the system with a taint
value.  In contrast, \quire's approach requires only the 
IPC subsystem be modified with no reliance on instrumented code,
therefore \quire can work with applications that use native
libraries and avoid the overhead imparted by instrumenting code to
propagate taint values.
\fi


\if 0
\subsection{Information flow control}
The idea of tracking and annotating the flow of information throughout
an operating system is not new.  Many existing information flow
control systems, such as JFlow~\cite{jflow}, use a combination of dynamic taint
tracking and tagged data to enforce security guarantees on the data
flowing through the system.  \quire differs from existing
information flow control systems in that it doesn't focus on
propagating taint but rather attempts to preserve the originator of a
request throughout the lifetime of a call chain.  \quire also
relies on process isolation and augments IPC channels to track provenance rather than relying on augmentations to an applications code to
propagate taint tags.

\subsection{Decentralized information flow control}
A branch of the information flow control space focuses on how to
provide taint tracking in the presence of mutually distrusting
applications and no centralized authority.  Meyer's and Liskov's work
on decentralized information flow control (DIFC)
systems~\cite{liskov-flowcontrol,meyers-difc} was the first attempt to
solve this problem.  Systems like DEFCon~\cite{defcon} and
Asbestos~\cite{asbestos} use DIFC mechanisms to dynamically apply
security labels and track the taint of events moving through a
distributed system.  These projects and \quire are similar in that
they both rely on process isolation and communication via message
passing channels that label data.  However, DEFCon cannot provide its
security guarantees in the presence of deep copying of data while
\quire can survive in an environment where deep copying is allowed
since \quire defines policy based on the call chain and ignores the
data contained within the messages forming the call chain.  Asbestos
avoids the deep copy problems of DEFCon by tagging data at the IPC
level.  
% 
% The tagging approach used in Asbestos was an inspiration for
% the IPC level tagging used in \quire.
% 
While Asbestos and \quire
use a similar approach to data tagging, the tags are used for very
different purposes.  Asbestos aims to prevent data leaks by enabling
an application to tag its data and disallow a recipient application
from leaking information that it received over an IPC channel while
\quire attempts to pre-emptively disallow data from being leaked by protecting
the resource itself, rather than allowing the resource to be accessed
then blocking leakage at the taint sink.
\fi

